Multimodal Machine Translation through Visuals and Speech

Multimodal machine translation involves drawing information from more than one modality, based on the assumption that the additional modalities will contain useful alternative views of the input data. The most prominent tasks in this area are spoken language translation, image-guided translation, and video-guided translation, which exploit audio and visual modalities, respectively. These tasks are distinguished from their monolingual counterparts of speech recognition, image captioning, and video captioning by the requirement of models to generate outputs in a different language. This survey reviews the major data resources for these tasks, the evaluation campaigns concentrated around them, the state of the art in end-to-end and pipeline approaches, and also the challenges in performance evaluation. The paper concludes with a discussion of directions for future research in these areas: the need for more expansive and challenging datasets, for targeted evaluations of model performance, and for multimodality in both the input and output space.

==> sections/models_igt_leftovers.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AN OLD PARAGRAPH that is almost integrated into the first paragraph below
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%An example in which the default machine translation assumptions are widened is multimodal machine translation (MMT), where the requirement is to have at least two different modalities (\emph{e.g.} text, audio, visuals) collectively pertaining to the source and target side. While this still allows many possible configurations, the typical configuration has text output as the target side, and the multimodality comes from a single non-text modality either augmenting or replacing the source text as the input.
%Table \ref{tab:mmt_overview} presents an overview of the different approaches in the literature. A tensor of visual features implies a volume of features ($\mathbb{R}^{x \times y \times z}$) that preserve \emph{spatial} information with respect to the original image; \emph{pooled} features ($\mathbb{R}^{v}$) are typically extracted from the penultimate layer of the original convolutional computer vision model; and \emph{objects} are typically discrete labelled regions in the original image. External textual data can be monolingual text or a parallel text, and external multimodal data is usually captioned images.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AN OLD PARAGRAPH that is not used so far
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%It should be noted that the best practices outlined above are for non-text modalities in isolation, while the best practice of encoding the entire multimodal input is still debated. In the multimodal MT literature, one group of studies seems to prefer employing multiple encoders for different modalities and letting the attention mechanism handle the rest~(\emph{e.g.}~\citet{libovicky-cuni-2016}), whereas another group is investigating ways to encode multimodal input jointly into the same latent space~(\emph{e.g.}~\citet{elliott-imagination-2017} and~\citet{zhou-visual-2018}), as shown in Figure~\ref{fig:mmt:approaches:visual-grounding}. For the former case, there are further questions of how to integrate the embeddings into the current MT architectures (see Figure~\ref{fig:mmt:approaches:plugging} for illustrative examples), and how to adapt attention to multivariate input (\emph{e.g.} by concatenating the input~\citep{huang-attention-based-2016}, employing separate attention heads~\citep{libovicky-cuni-2016}, or using hierarchical multi-layered attention~\citep{moon-multimodal-2018}). For the latter case, the translation architecture learns to ground knowledge between the modalities, which is only meaningful when the different modalities describe different aspects of one notion (\emph{e.g.} an image and its description, but not a video clip and subtitles). 

% Training a deep learning model to perform multiple tasks at once can improve the model's general performance at those by forcing the model to represent shared knowledge in a broader sense, as long as the objectives of the tasks are relevant for each other. While the idea has been implemented for multimodal MT in \emph{e.g.} Elliott and Kádár's Imagination architecture~\citep{elliott-imagination-2017}~(see Figure~\ref{fig:mmt:approaches:imagination}), it is not nearly as well-studied as in text-based multilingual MT~(\emph{e.g.}~\citet{johnson-googles-2016}). Furthermore, recent studies of compound attention~\citep{cifka-are-2018,vazquez-multilingual-2018} described attempts to reinstate the aggregate sequence embedding point between the encoder and the decoder, and as a good side effect, they may have provided a mechanism for efficiently learning to attend to multiple aspects of the same input data. This could be used to encode \emph{e.g.} both text and images into the same shared intermediate representation and enable a multi-task training schedule that simultaneously learns to caption images and (unimodally) translate captions, possibly bootstrapping an effective multimodal caption translation model.
